Computational analysis of interface evolution and droplet pinch-off mechanism in two-phase liquid flow through T-junction microfluidic system

This work has explored interface evolution and pinch-off mechanism of the droplet formation in two-phase flow through cross-flow microfluidic device. The two-dimensional mathematical model equations have been solved using the finite element method under the squeezing regime ($Ca_c < 10^{-2}$) for wide range of flow rates ($Qr = 0.1 - 10$) and fixed contact angle ($\theta=135^o$). The droplet formation process has been classified into various instantaneous stages as initial, filling, squeezing, pinch-off and stable droplet through microscopic visualization of interface evolution in phase profiles. The dynamics of interface, and point pressure in both phases is further gained and discussed. Maximum pressure in the continuous phase varied linearly with Qr. The droplet pinch-off mechanism has been thoroughly elucidated by determining the local radius of the curvature ($R_{c,min}$) and neck width (2r) during the squeezing and pinch-off stages. At the pinch-off point, both $R_{c,min}$ and 2r are non-linearly related to Qr. Further, the topological dynamics of interface has been explored by analyzing the Laplace pressure ($p_{\text{L}}$), acting on the interface curvature, evaluated using (a) pressure sensors in both phases, (b) local radius of curvature, and (c) minimum radius of curvature. The insights obtained from the present work can reliably be used in designing the model and prototypes of microfluidic devices for generating monodispersed droplets in emulsions, and the droplet breakup mechanism would help accurate prediction of the pinch-off moment. The proposed knowledge provides detailed insights of the interface evolution and droplet pinch-off to a precision of 10 $\mu$s and resolution of 10 $\mu$m, equivalent to experimental flow visualization with a high-speed ($10^{5}$ fps) and high-resolution (10 $\mu$m pixel size) camera.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~




==> makeglossaries <==
#!/usr/bin/env perl

# File    : makeglossaries
# Author  : Nicola Talbot
# Version : 4.45
# Description: simple Perl script that calls makeindex or xindy.
# Intended for use with "glossaries.sty" (saves having to remember
# all the various switches)

# This file is distributed as part of the glossaries LaTeX package.
# Copyright 2019 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

# This work consists of the files glossaries.dtx and glossaries.ins 
# and the derived files glossaries.sty, glossaries-prefix.sty,
# glossary-hypernav.sty, glossary-inline.sty, glossary-list.sty, 
# glossary-long.sty, glossary-longbooktabs.sty, glossary-longragged.sty,
# glossary-mcols.sty, glossary-super.sty, glossary-superragged.sty, 
# glossary-tree.sty, glossaries-compatible-207.sty, 
# glossaries-compatible-307.sty, glossaries-accsupp.sty, 
# glossaries-babel.sty, glossaries-polyglossia.sty, glossaries.perl.
# Also makeglossaries and makeglossaries-lite.lua.

my $version="4.45 (2020-01-18)";

# History:
# v4.43:
#   * No change.
# v4.41:
#   * No change.
# v4.40:
#   * No change.
# v4.39:
#   * No change.
# v4.38:
#   * No change.
# v4.37:
#   * No change.
# v4.36:
#   * No change.
# v4.35:
#   * No change.
# v4.34:
#   * Added check for \glsxtr@resource
# v4.33:
#   * Version number synchronized with glossaries.sty
# v2.21:
#   * Fixed spelling of \GlsAddXdyLocation
#   * Adjusted range encap clash
# v2.20 (2016/12/16)
#   * Added check for \glsxtr@makeglossaries
# v2.19 (2016/05/27)
#   * Improved check in &parse_for_xindy_nosort
# v2.18 (2016/01/24)
#   * Added &parse_for_xindy_nosort to help diagnose xindy's empty
#     index key warning/error.
#   * Added check for makeindex's multiple encap warning.
# v2.17 (2015/11/30)
#   * Escaped { in regular expressions.
#     http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=101
# v2.16 (2015/06/28)
#   * Added check for "german" and codepage that doesn't contain
#   "din5007", "duden" or "braille". If missing, "din5007-" is
#   prefixed to the codepage.
# v2.15 (2014/07/30)
#   * Removed hard-coded three character extension assumption
#     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=55
#   * Added message to indicate the number of ignored glossaries
#     when the extension is specified.
# v2.14 (2014/03/06)
#   * Added -Q and -k options
# v2.13 (2014/01/21)
#   * Added check for leading and trailing quotes in filename
# v2.12 (2014/01/20)
#   * Added check for '*' in istfilename
#   * Fixed bug report
#   http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=33
#   * Added error text hashes
# v2.11 (2014/01/17):
#   * Added check for backslashes in -x, -m and -d paths
#   * Added double-quotes around $appname in &run_app
# v2.10 (2013/12/01):
#   * initialise $language to suppress warnings
# v2.09 (2013-11-12):
#   * added check for -q switch when issuing warnings.
# v2.08 (2013-10-14):
#   * added -x and -m options
# v2.07 (2013-06-17):
#   * added check for success on chdir if -d used
#   * added dialect map
# v2.06 (2013-04-21):
#   * added "din5007" as default if language is set to "german"
# v2.05 (2012-11-12):
#   * added -d option
# v2.04 (2012-04-19):
#   * fixed bug in &scan_aux
# v2.03 (2011-04-12):
#   * added warning about possibly needing 'nomain' package option
# v2.02 (2011-04-2):
#   * Prints version number at start of run unless -q
#   * Added more diagnostics.
# v2.01 (2010-09-29):
#   * Added 'use warnings'
# v2.0 (2010-06-30) :
#   * Made file handle local in &scan_aux
# v1.9 (2010-06-14) :
#   * Check for \@input
# v1.8 (2009-11-03) :
#   * Create an empty output file if the input file is empty
#     without calling xindy/makeindex
# v1.7 (2009-09-23) :
#   * Issue warning rather than error when empty/non existant file 
#     checks fail
# v1.6 (2009-05-24) :
#   * main glossary no longer automatically added
#     (only added if information in aux file)
#   * if file extension is specified, check added to ensure it
#     corresponds to a known glossary extension.
#   * added file existance test and file empty test
# v1.5 (2008-12-26) :
#   * added support for xindy
#   * picks up ordering information from aux file
# v1.4 (2008-05-10) :
#   * added support for filenames with spaces.
# v1.3 (2008-03-08) :
#   * changed first line from /usr/bin/perl -w to /usr/bin/env perl
#     (Thanks to Karl Berry for suggesting this.)
# v1.2 (2008-03-02) :
#   * added support for --help and --version
#   * improved error handling
# v1.1 (2008-02-13) :
#   * added -w and strict
#   * added check to ensure .tex file not passed to makeglossaries
#
# v1.0 (2007-05-10) : Initial release.

use Getopt::Std;
use strict;
# v2.01 added the following line
use warnings;
# v2.05 added $opt_d
# v2.08 added $opt_x and $opt_m
use vars qw($opt_q $opt_t $opt_o $opt_s $opt_p $opt_g $opt_c $opt_r
   $opt_l $opt_i $opt_L $opt_n $opt_C $opt_d $opt_x $opt_m $opt_Q
   $opt_k);


$Getopt::Std::STANDARD_HELP_VERSION = 1;

# v1.5 added -L <lang> for xindy (but language can be specified in 
# .tex file)
# v1.5 added -n (print the command that would be issued but
# don't actually run the command)
getopts('s:o:t:p:L:C:ilqQkrcgnd:x:m:');

unless ($#ARGV == 0)
{
   die "makeglossaries: Need exactly one file argument.\n",
       "Use `makeglossaries --help' for help.\n";
}

# v2.02: added:
print "makeglossaries version $version\n" unless ($opt_q);

# v2.07: added babel dialect -> xindy language map:
my %languagemap =
(
  'american'  => 'english',
  'austrian'  => 'german',
  'british'   => 'english',
  'francais'  => 'french',
  'frenchb'   => 'french',
  'germanb'   => 'german',
  'lsorbian'  => 'lower-sorbian',
  'magyar'    => 'hungarian',
  'naustrian' => 'german',
  'ngermanb'  => 'german',
  'ngerman'   => 'german', # v2.16
  'norsk'     => 'norwegian',
  'portuges'  => 'portuguese',
  'russianb'  => 'russian',
  'slovene'   => 'slovenian',
  'UKenglish' => 'english',
  'USenglish' => 'english',
  'ukraineb'  => 'ukrainian',
  'usorbian'  => 'upper-sorbian'
);

# v2.07 added check for success and for -q
# v2.05 added:

if ($opt_d)
{
  # v2.11 check for backslash character if on Windows
  $opt_d=~s/\\/\//g if $^O=~/Win/;

  if (chdir $opt_d)
  {
     print "Changed to '$opt_d'\n" unless ($opt_q);
  }
  else
  {
     die "Unable to chdir to '$opt_d' $!\n";
  }
}

# v2.02: added:
# v2.19: changed value
my $xdynotist = 2;
# v2.13: removed
#my $needcompatibilitymode=2;

# v2.13: added $istnotfound
my $istnotfound = 3;

# v2.13: added error text:
my %makeindex_error_text =
 (
   $xdynotist => "Style name indicates makeindex, but may be in xindy format.\n"
          . "Remember to use \\setStyleFile to specify the name\n"
          . "of the style file rather than redefining \\istfilename\n"
          . "explicitly.",
   $istnotfound => "Style file not found. (Have you used \\noist by mistake?)"
 );

my %xindy_error_text =
 (
   'nosort'    => "Sort key required for entries only containing command names.",
   'istnotxdy' =>
      "Style name has xdy extension, but may be in makeindex format.\n"
     . "Remember to use \\setStyleFile to specify the name\n"
     . "of the style file rather than redefining \\istfilename\n"
     . "explicitly.",
   'missingendquote' =>
       "You may have missed a \" character in a command such as \\GlsAddXdyLocation.",
    'nolanguage' =>
       "No language detected.\nHave you remembered to use \\printglossary\n".
       "or \\printglossaries in your document?",
    'nomain' =>
        "\nRemember to use package option 'nomain' if you don't\n".
        "want to use the main glossary.",
#v2.21: fixed spelling of \GlsAddXdyLocation
    'badlocation' =>
        "You may have forgotten to add a location \n"
        . "class with \\GlsAddXdyLocation or you may have \n"
        . "the format incorrect.\n",
    'comp207' => "You may need to add 'compatible-2.07' package option.",
    'noxdyfile' => "Style file not found. (Have you used \\noist by mistake?)"
 );

# define known extensions

# v1.6: removed adding main glossary here as there's no guarantee
# that it's been used. If it has been used, the information will
# be picked up later in the aux file
my %exttype = (
#   main => {in=>'glo', out=>'gls', 'log'=>'glg'},
 );

# v1.5 define require languages for xindy

my %language = ();
my %codepage = ();

my $ext = '';
my $name = $ARGV[0];

# v2.13 added:
#$name=~s/^"(.*)"$/$1/;
# v2.15: fix provided by Herb Schulz to allow for extensions that
# aren't exactly three characters:
# (HS) changes fix for 3 character extension limit
my ($basename,$extension) = ($name =~ m/^(.*?)(?:\.([^\.]*))?$/);
# (HS) end of changes fix for 3 character extension limit

# make sure $extension is defined. (If there was no match in the
# above, it cause an uninitialised error later.)
$extension = '' unless ($extension);

# Make sure users don't try passing the tex file:

#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
# (HS) changes fix for 3 character extension limit
#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
  if (lc($extension) eq 'tex')
  {
     die("Don't pass the tex file to makeglossaries:\n"
        ."either omit the extension to make all the glossaries, "
        ."or specify one of the glossary files, e.g. $name.glo, to "
        ."make just that glossary.\n")
  }
#}
# (HS) end of fix for 3 character extension limit

# (HS) changes fix for 3 character extension limit
$ext = $extension;
$name = $basename;
# (HS) end of changes fix for 3 character extension limit

# v2.01 add check to see if aux file exists

unless (-e "$name.aux")
{
   die "Auxiliary file '$name.aux' doesn't exist. Have you run LaTeX?\n";
}

my $istfile = "";

my $glslist = "";

# should letter ordering be used? (v1.5 added)

my $letterordering = defined($opt_l);

# v2.19 added:
my $extramkidxopts = '';

# v4.34 added:
my $foundbib2glsresource = '';

# Check aux file for other glossary types,
# style file name and various other bits of information.

&scan_aux($name);

# has the style file been specified?
unless ($istfile)
{
   if ($foundbib2glsresource)
   {
      die "Found \\glsxtr\@resource in '$name.aux',\n",
          "but not found \\\@istfilename.\n",
          "You need to run bib2gls not makeglossaries.\n";
   }
   else
   {
      die "No \\\@istfilename found in '$name.aux'.\n",
          "Did your LaTeX run fail?\n",
          "Did your LaTeX run produce any output?\n",
          "Did you remember to use \\makeglossaries?\n";
   }
}

# v2.08 added $xindyapp and $makeindexapp
# By default assume they are on the operating system's path
my $xindyapp = ($opt_x ? $opt_x :'xindy');
my $makeindexapp = ($opt_m ? $opt_m :'makeindex');

# v2.11 check for backslash character if on Windows
if ($^O=~/Win/)
{
  $xindyapp=~s/\\/\//g;
  $makeindexapp=~s/\\/\//g;
}

# v1.5 save the general xindy switches

my $xdyopts = '';

# v2.01 replaced 'unless ($opt_L eq "")' with 'if ($opt_L)'
if ($opt_L)
{
  $xdyopts .= " -L $opt_L";
}

# save all the general makeindex switches

my $mkidxopts = '';

if ($opt_i)
{
   $mkidxopts .= " -i";
}

if ($letterordering)
{
   $mkidxopts .= " -l";
   $xdyopts .= " -M ord/letorder";
}

if ($opt_q)
{
# v2.01 removed following lines. (This script now deals with
# printing messages to STDOUT.)
   #$mkidxopts .= " -q";
   #$xdyopts .= " -q";
}

if ($opt_r)
{
   $mkidxopts .= " -r";
}

if ($opt_c)
{
   $mkidxopts .= " -c";
}

if ($opt_g)
{
   $mkidxopts .= " -g";
}

# v2.01 replaced 'unless ($opt_p eq "")' with 'if ($opt_p)'
if ($opt_p)
{
   $mkidxopts .= " -p $opt_p";
}

if ($extramkidxopts)
{
  $mkidxopts .= " $extramkidxopts";
}

# v2.01 replaced 'unless ($opt_s eq "")' with 'if ($opt_s)'
if ($opt_s)
{
   # v2.01 check if user has specified -s <file>.ist but aux file
   # indicates .xdy ought to be used and vice-versa. Also check if
   # requested style file exists

   unless (-e $opt_s)
   {
      die "\n",
         "Requested style file '$opt_s' doesn't exist.\n\n";
   }

   if ($istfile=~/\.xdy$/ and $opt_s!~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using xindy,\n",
        "but you have specified makeindex style file '$opt_s'\n",
        "Make sure you don't specify 'xindy' as a package option if\n",
        "you want to use makeindex.\n\n",
        "\\usepackage[makeindex]{glossaries}\n\n";
   }
   elsif ($istfile!~/\.xdy$/ and $opt_s=~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using\n",
        "makeindex, but you have specified xindy style file '$opt_s'.\n",
        "Make sure you specify 'xindy' as a package option if you\n",
        "want to use xindy.\n\n",
        "\\usepackage[xindy]{glossaries}\n\n";
   }

   $istfile = $opt_s;
}

# Use xindy if style file ends with .xdy otherwise use makeindex

my $usexindy = ($istfile=~m/\.xdy\Z/);

if ($ext)
{
   # an extension has been specified, so only process
   # the specified file

   # v1.6 %thistype is no longer given a default value
   my %thistype;

   my $thislang = "";
   my $thiscodepage = "";

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      if ($exttype{$type}{'in'} eq $ext)
      {
         %thistype = %{$exttype{$type}};

         $thislang = $language{$type};

         $thiscodepage = $codepage{$type};

         last;
      }
   }

   # v1.6 If %thistype hasn't been defined, then the given
   # extension doesn't correspond to any known glossary type

   # v2.01 replaced deprecated 'defined(%thistype)' with %thistype
   unless (%thistype)
   {
      die "The file extension '$ext' doesn't correspond to any\n",
          "known glossary extension. Try running makeglossaries\n",
          "without an extension, e.g. makeglossaries \"$name\".\n";
   }

   my $outfile;

# v2.01 replaced 'if ($opt_o eq "")' with 'unless ($opt_o)'
   unless ($opt_o)
   {
      $outfile = "$name.$thistype{out}";
   }
   else
   {
      $outfile = $opt_o;
   }

   my $transcript;

# v2.01 replaced 'if ($opt_t eq "")' with 'unless ($opt_t)'
   unless ($opt_t)
   {
      $transcript = "$name.$thistype{'log'}";
   }
   else
   {
      $transcript = $opt_t;
   }

# v2.01 remove old transcript file

   unless ($opt_n)
   {
      unlink($transcript);
   }

   if ($usexindy)
   {
      &xindy("$name.$ext", $outfile, $transcript,$istfile,
        $thislang, $thiscodepage, $xdyopts, $opt_q, $opt_n, $xindyapp);
   }
   else
   {
      &makeindex("$name.$ext",$outfile,$transcript,$istfile,
                 $mkidxopts,$opt_q, $opt_n, $makeindexapp, 1);
   }


   # v2.15 added:

   my $num_omitted = $#types;

   if ($num_omitted == 1)
   {
      print "1 glossary ignored.\n" unless $opt_q;
   }
   elsif ($num_omitted > 1)
   {
      print "$num_omitted glossaries ignored.\n" unless $opt_q;
   }
}
else
{
   # no file extension specified so process all glossary types

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      my %thistype = %{$exttype{$type}};

      my $inputfile = "$name.$thistype{in}";

      my $outfile;

# v2.01 changed 'if ($opt_o eq "")' with 'unless ($opt_o)'
      unless ($opt_o)
      {
         $outfile = "$name.$thistype{out}";
      }
      else
      {
         $outfile = $opt_o;
      }

      # v1.7 print warnings to STDOUT instead of STDERR

      # v1.6 added file existence test
      unless (-e $inputfile)
      {
         # v2.09 suppress warning if -q switch in use
         print "Warning: File '$inputfile' doesn't exist.\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      unless (-r $inputfile)
      {
         print "Warning: No read access for '$inputfile' $!\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      my $transcript;

# v2.01 changed 'if ($opt_t eq "")' with 'unless ($opt)'
      unless ($opt_t)
      {
         $transcript = "$name.$thistype{'log'}";
      }
      else
      {
        $transcript = $opt_t;
      }

      # v1.6 added file empty test
      if (-z $inputfile)
      {
         my $message =
             "Warning: File '$inputfile' is empty.\n".
             "Have you used any entries defined in glossary '$type'?\n";

         if ($type eq 'main')
         {
            $message .=
               "Remember to use package option 'nomain' if you\n".
               "don't want to use the main glossary.\n";
         }

         # v2.09 suppress warning if -q switch in use
         warn $message unless $opt_q;

         # Write warning to transcript file.

         if (open TRANSFD, ">$transcript")
         {
            print TRANSFD $message;
            close TRANSFD;
         }

         # create an empty output file and move on to the next glossary

         if (open OFD, ">$outfile")
         {
            print OFD "\\null\n";
            close OFD;
         }
         else
         {
            warn "Unable to create '$outfile' $!\n";
         }

         next;
      }

# v2.01 remove old transcript file

      unless ($opt_n)
      {
         unlink($transcript);
      }

      if ($usexindy)
      {
         &xindy($inputfile,$outfile,$transcript,$istfile,
                $language{$type},$codepage{$type},
                $xdyopts,$opt_q,$opt_n, $xindyapp);
      }
      else
      {
         &makeindex($inputfile,$outfile,$transcript,
                    $istfile,$mkidxopts,$opt_q,$opt_n, $makeindexapp, 1);
      }
   }
}

sub scan_aux{
  my $name = shift;

  # v2.0 added
  local(*AUXFILE);

  if (open AUXFILE, "$name.aux")
  {
     while (<AUXFILE>)
     {
        #v2.14 added
        if (m/\\\@gls\@reference/ and not $glslist)
        {
           die "Your document has used \\makenoidxglossaries\n",
               "You don't need makeindex or xindy.\n";
        }

        if (m/\\glsxtr\@makeglossaries\{(.*)\}/)
        {
           #v2.20 added

           $glslist = $1;

           unless ($opt_q)
           {
              print "only processing subset '$glslist'\n";
           }
        }
        elsif (m/\\\@input\{(.+)\.aux\}/)
        {
           # v1.9 added
           # v2.17 escaped { in regex
           &scan_aux($1);

           # v2.04 added
           # (Fix provided by Daniel Grund) 
           next;
        }
        elsif (m/\\\@newglossary\s*\{(.*)\}\{(.*)\}\{(.*)\}\{(.*)\}/)
        {
           # v2.17 escaped { in regex

           $exttype{$1}{'log'} = $2;
           $exttype{$1}{'out'} = $3;
           $exttype{$1}{'in'}  = $4;

           unless ($opt_q)
           {
              print "added glossary type '$1' ($2,$3,$4)\n";
           }
        }
        elsif (m/\\\@istfilename\s*\{([^}]*)\}/)
        {
           # v2.17 escaped { in regex

           $istfile = $1;

           # check if double quotes were added to \jobname
           # v2.12 added check for xdy (bug ID 33)
           $istfile=~s/^"(.*)"\.(ist|xdy)$/$1.$2/;

           # v2.12 if on Windows, substitute any '*' with ' '
           # to compensate for MiKTeX bug
           # http://sourceforge.net/p/miktex/bugs/2301/

           if ($^O=~/Win/)
           {
              $istfile=~tr/\*/ /;
           }
        }
        elsif (m/\\\@xdylanguage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $language{$1} = $2;
        }
        elsif (m/\\\@gls\@codepage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $codepage{$1} = $2;
        }
        elsif (m/\\\@gls\@extramakeindexopts\{(.*)\}/)
        {
           # v2.19 added

           $extramkidxopts .= $1;
        }
        elsif (m/\\glsxtr\@resource/)
        {
           # v4.34 added

           # No error at this point as a hybrid method is allowed.
           # Error only occurs if no \@istfilename found.

           $foundbib2glsresource = 1;
        }

        # v1.5 added
        # Allow -l switch to override specification in aux file
        unless (defined($opt_l))
        {
           # v2.17 escaped { in regex
           if (m/\\\@glsorder\s*\{([^}]+)\}/)
           {
              my $ordering = $1;

              if ($ordering eq "word")
              {
                 $letterordering = 0;
              }
              elsif ($ordering eq "letter")
              {
                 $letterordering = 1;
              }
              else
              {
                 warn
                   "Unknown ordering '$ordering'\n",
                   "Assuming word ordering\n" unless ($opt_q);
                 $letterordering = 0;
              }
           }
        }
     }

     close AUXFILE;
  }
  else
  {
     warn "Unable to open $name.aux: $!\n";
  }
}

# v2.01 new subroutine run_app added
sub run_app{
   my($appname, $appargs, $trans, $quiet, $dontexec) = @_;

   local(*STATUS);

   my $status   = '';
   my $warnings = '';
   my $errno = 0;
   my $log = '';

   print "$appname $appargs\n" if ($dontexec or not $quiet);

   return if ($dontexec);

   # v2.11 added double-quotes around $appname
   # v2.14 added -k switch
   if (not $opt_k and open (STATUS, "\"$appname\" $appargs 2>&1 |"))
   {
      while (<STATUS>)
      {
         print unless ($quiet);

         $warnings .= $_ if (/WARNING:/);

         $status .= $_ unless (/^[\w]+ing/ or /^Finished/ or /^Usage:/);

         $log .= $_;
      }

      close STATUS;
   }
   else
   {
      unless ($opt_k)
      {
         $warnings = "Unable to fork \"$appname\" with redirection $!\n";

         # v2.14 added check for quiet switches
         warn $warnings,  
           "Retrying without redirection.\n" unless ($quiet or $opt_Q);
      }

      $status = `\"$appname\" $appargs`;

      $log = $status;

      print $status unless ($quiet);
   }

   if ($?)
   {
      # v2.14 Fixed error number assignment
      $errno = ($? >> 8);

      # v2.14 Added check for existence of transcript
      unless (-e $trans)
      {
         $log .= "\n$appname didn't create a transcript.\n";

         if (not $appname=~/\//)
         {
            # No path specified
            $log .= "Check that $appname has been installed and\nis on your system's PATH.\n";

            if (defined $ENV{PATH})
            {
               $log .= "Your PATH environment variable is set to: \n"
                    . $ENV{PATH} . "\n";
            }
            else
            {
               $log .= "I'm sorry, I can't detect your PATH environment variable\n";
            }

            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
         elsif (not -e $appname)
         {
            if ($^O=~/Win/)
            {
               if (-e "$appname.exe" or -e "$appname.bat")
               {
                  $log .= "Try manually running:\n\"$appname\" $appargs\n";
               }
               else
               {
                  $log .= "File '$appname' doesn't exist.\n";
               }
            }
            else
            {
               $log .= "File '$appname' doesn't exist.\n";
            }
         }
         else
         {
            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n\n*** Unable to execute: '\"$appname\" $appargs' ***\n\n";
         print LOGFILE "Failed with error code $errno.\n\n";

         if ($log)
         {
            print LOGFILE "Status report:\n\n";
            print LOGFILE "$log", "\n";
         }

         print LOGFILE "Warnings:\n\n",$warnings, "\n" if $warnings;
         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }

   if ($log=~/\(0 entries accepted,/
    or ( ($log=~/(\d+) warnings?/ and $1 gt 0))
    or $log=~/not found/)
   {
      # Attempt to diagnose what's gone wrong

      if (open TRANS, $trans)
      {
         while (<TRANS>)
         {
            if (/Index style file .* not found/)
            {
               $errno = $istnotfound;
               last;
            }
            elsif (/Unknown specifier ;/)
            {
               $errno = $xdynotist;
               last;
            }
            elsif (/## Warning \(.*\):\s*$/)
            {
               $warnings .= $_ . <TRANS>;
            }
         }

         close TRANS;
      }

   }

   return ($status, $warnings, $errno);
}

# v2.08 added $app parameter
sub makeindex{
   my($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,$repairencaps) = @_;

   my $args = "$rest -s \"$ist\" -t \"$trans\" -o \"$out\" \"$in\"";

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($errno)
   {
      my $diagnostic = '';

      if ($makeindex_error_text{$errno})
      {
         $diagnostic = $makeindex_error_text{$errno};
      }
      else
      {
         $diagnostic = "Can't find diagnostic message for error code $errno";
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to makeindex failed***\n", 
        ($diagnostic ?
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"
        ),
        "Check '$trans' for details\n";
   }

   # 2.18: added check and repair for multiple encaps
   if ($warnings)
   {
      warn $warnings unless $quiet;

      if ($repairencaps and $warnings=~/multiple encaps/)
      {
         unless ($quiet)
         {
            print "Multiple encaps detected. Attempting to remedy.\n";
            print "Reading $in...\n";
         }

         # if $in can't be opened at this point something wrong
         # has occurred (otherwise how did makeindex manage to open
         # it?)

         open INFD, $in or die "Can't open '$in' $!\n";

         my @entries = ();

         while (<INFD>)
         {
            if (/\\glossaryentry\{(.*)\|([^\|]*)\}\{(.*?)\}/)
            {
               my %entry = 
                (
                   'entry' => $1,
                   'encap' => $2,
                   'location' => $3
                );

               my $add = 1;

               for (my $idx = 0; $idx <= $#entries; $idx++)
               {
                  my $existing = $entries[$idx];

                  if ($entry{'entry'} eq $existing->{'entry'}
                  and $entry{'location'} eq $existing->{'location'}
                  and $entry{'encap'} ne $existing->{'encap'})
                  {
                     $add = 0 if ($add == 1);

                     # Range encaps should take precedence.

                     if ($entry{'encap'}=~/^[\(\)]/)
                     {
                        $add = 2;

                        if ($existing->{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           last;
                        }
                        else
                        {
                           # remove existing

                           splice @entries, $idx, 1;

                           $idx--;
                        }
                     }
                     elsif ($existing->{'encap'}=~/^[\(\)]/)
                     {
                        if ($entry{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           $add = 1;
                           last;
                        }
                        # (otherwise drop new entry)
                     }
                     elsif (&encap_overrides($entry{'encap'},
                                   $existing->{'encap'}))
                     {
                        $entries[$idx] = \%entry;
                     }
                  } 
               }

               push @entries, \%entry if $add > 0;
            }
            else
            {
               warn "Abandoning attempt. Can't parse: $_" unless $quiet;

               close INFD;
               return;
            }
         }

         close INFD;

         if (open OUTFD, ">$in")
         {
            print "Writing $in...\n" unless $quiet;

            foreach my $entry (@entries)
            {
               print OUTFD '\\glossaryentry{',
                 $entry->{'entry'}, '|',
                 $entry->{'encap'}, '}{',
                 $entry->{'location'}, '}', "\n";
            }

            close OUTFD;

            print "Retrying\n" unless $quiet;

            &makeindex($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,0);
         }
         else
         {
            warn "Can't open '$in' $!\n" unless $quiet;
         }
      }
   }
}

# 2.18 new
# This is a subroutine in case of possible extension.
# For example, what happens in the event of 'textbf' and 'emph'?
# Should one override the other or be combined? Combining is harder
# as it would need a corresponding LaTeX command. (bib2gls deals
# with this better through its --map-formats switcn.)
# 2.21 check for range encap moved earlier

sub encap_overrides{
  my ($newencap, $existing) = @_;

  ($existing=~/\\glsnumberformat\s*$/ or $newencap!~/\\glsnumberformat\s*$/ )
}

# v2.08 added $app parameter
sub xindy{
   my($in,$out,$trans,$ist,$language,$codepage,$rest,$quiet,
     $dontexec, $app) = @_;
   my($args, $langparam, $main, $retry);
   my($module);

   $module = $ist;
   $module=~s/\.xdy\Z//;

   if ($language)
   {
     # map babel names to xindy names

     $language = $languagemap{$language} if ($languagemap{$language});

     $langparam = "-L $language";
   }
   else
   {
     $langparam = "";
     # v2.10 initialise $language to suppress warnings
     $language = "";
   }

   # most languages work with xindy's default codepage, but
   # some don't, so if the codepage isn't specific, check
   # the known cases that will generate an error
   # and supply a default. (For all other cases, it's up to the 
   # user to supply a codepage.)

# v2.01 changed 'if ($codepage eq "")' to 'unless ($codepage)'
   unless ($codepage)
   {
      if ($language eq 'dutch')
      {
         $codepage = "ij-as-ij";
      }
      elsif ($language eq 'german')
      {
         $codepage = "din5007";
      }
      elsif ($language eq 'gypsy')
      {
         $codepage = "northrussian";
      }
      elsif ($language eq 'hausa')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'klingon')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'latin')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'mongolian')
      {
         $codepage = "cyrillic";
      }
      elsif ($language eq 'slovak')
      {
         $codepage = "small";
      }
      elsif ($language eq 'spanish')
      {
         $codepage = "modern";
      }
      elsif ($language eq 'vietnamese')
      {
         $codepage = "utf";
      }
   }
   elsif ($language eq 'german' and $codepage!~/(din5007|duden|braille)/)
   {
#v2.16 added check for german din/duden

      $codepage = "din5007-$codepage";
   }


   my $codepageparam = "";

   if ($codepage)
   {
      $codepageparam = "-C $codepage";
   }

   $main = join(' ',
      "-I xindy",
      "-M \"$module\"",
      "-t \"$trans\"",
      "-o \"$out\"",
      "\"$in\"");

   $args = join(' ', $rest, $langparam, $codepageparam, $main);

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($status=~/Cannot locate xindy module for language ([^\s]+) in codepage ([^\s]+)/)
   {
      $args = join(' ', $rest, $langparam, $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying using default codepage.\n";

         warn $message;

         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($status=~/Cannot locate xindy module for language ([^\s]+)/
    and $1 ne 'general')
   {
      $args = join(' ', $rest, "-L general", $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying with -L general\n";

         warn $message;
         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($errno)
   {
      # attempt further diagnostic

      my $diagnostic = '';

      if ($status=~/index 0 should be less than the length of the string/m)
      {
         $diagnostic = $xindy_error_text{nosort};

         $diagnostic .= &parse_for_xindy_nosort($in);
      }
      elsif ($status=~/variable .+ has no value/m)
      {
         # v2.19 fixed misspelt key
         $diagnostic = $xindy_error_text{istnotxdy};
      }
      elsif ($status=~/Could not find file /m)
      {
         # v2.19 added
         $diagnostic = $xindy_error_text{noxdyfile};
      }
      elsif ($status=~/Possible read-error due to ill-formed string " :sep/m)
      {
         $diagnostic = $xindy_error_text{missingendquote};
      }
      elsif (not $language)
      {
         # If the language hasn't been set, then it may be
         # because the document doesn't contain
         # \printglossaries/\printglossary or it may be
         # because the user has a customized style file that
         # contains the language settings.

          $diagnostic = $xindy_error_text{nolanguage};

          if ($in eq 'glo')
          {
             # or it may be that the user doesn't want to use the main
             # glossary and has forgotten to suppress it with the
             # "nomain" package option

             $diagnostic .= $xindy_error_text{nomain};
          }
      }

      # v2.19 added:
      if ($diagnostic and open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to xindy failed***\n", 
          ($diagnostic ? 
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"),
          "Check '$trans' for details\n";
   }

   # Check xindy warnings

   if ($status=~/^WARNING:/m)
   {
      my $diagwarn = '';

      if ($status=~/did not match any location-class/m)
      {
         $diagwarn = $xindy_error_text{badlocation};
      }

      if ($status=~/unknown attribute `pageglsnumberformat'/m)
      {
         $diagwarn .= $xindy_error_text{comp207};
      }

      if ($status=~/Would replace complete index key by empty string, ignoring/m)
      {
         $diagwarn .= $xindy_error_text{nosort};
         $diagwarn .= &parse_for_xindy_nosort($in);
      }

      if ($diagwarn)
      {
         warn "\n**Warning:**\n\n", $diagwarn, "\n";

         $warnings .= "\nmakeglossaries diagnostic messages:\n\n"
                   . $diagwarn;
      }
   }

   if ($retry or $warnings)
   {
      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n$warnings";

         if ($retry)
         {
            print LOGFILE "\nmakeglossaries messages:\n\n", $retry;
         }

         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }
}

# v2.18 added:
sub parse_for_xindy_nosort{
  my ($in) = @_;

  my $msg = join("\n", "", 
                 "Attempting to determine which entries have problem sort keys.",
                 "Parsing '$in'");

  my %entries = ();

  if (open FD, $in)
  {
     while (<FD>)
     {
# v2.19 extra conditions added
        if (/:tkey \(\("((?:\\\\[a-zA-Z@]+ *)+)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $label;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/([\\\s]+)//g;

           }
        }
        elsif (/:tkey \(\("(\\\\[a-zA-Z@]+ *{(?:\\\\[a-zA-Z@]+ *)+})+" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form \cs{\cs}
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
        elsif (/:tkey \(\("(\$\s*(?:\{?\\\\[a-zA-Z@]+ *\}?)+\$)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form $\cs$
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
     }

     close FD;

     my @labels = keys %entries;

     my $n = $#labels+1;

     if ($n == 0)
     {
        $msg .= "\nCouldn't find anything! Sorry, I'm stumped.";
     }
     else
     {
        $msg .= ($n == 1 ? "\n1 problematic entry found:\n"
                         : "\n$n problematic entries found:\n");

        foreach my $label (@labels)
        {
           my $thisentry = $entries{$label};

           $msg .= "\nLabel: '$label'. Sort value : '$thisentry->{sort}'";
           $msg .= "\n(Try adding sort={$thisentry->{suggestion}} to the definition.)";
        }
     }
  }
  else
  {
     $msg .= "\nFailed to open '$in' $!\n";
  }

  $msg;
}

sub HELP_MESSAGE{
   print "\nSyntax : makeglossaries [options] <filename>\n\n";
   print "For use with the glossaries package to pass relevant\n";
   print "files to makeindex or xindy.\n\n";
   print "<filename>\tBase name of glossary file(s). This should\n";
   print "\t\tbe the name of your main LaTeX document without any\n";
   print "\t\textension.\n";
   print "\nGeneral Options:\n\n";
   print "-o <gls>\tUse <gls> as the output file.\n";
   print "\t\t(Don't use -o if you have more than one glossary.)\n";
   print "-q\t\tQuiet mode.\n";
   print "-Q\t\tSilence unable to fork warning.\n";
   print "-k\t\tDon't try to use piped redirection.\n";
   print "-l\t\tLetter ordering.\n";   
   print "-s <sty>\tEmploy <sty> as the style file.\n";
   print "-t <log>\tEmploy <log> as the transcript file.\n";
   print "\t\t(Don't use -t if you have more than one glossary\n";
   print "\t\tor the transcripts will be overwritten.)\n";
   print "-d <directory>\tDirectory in which the .aux, .glo etc files are located.\n",
     "\t\t(Default is the directory in which <filename> resides.)\n";
   print "-n\t\tPrint the command that would normally be executed,\n",
         "\t\tbut don't execute it.\n";

   print "\nXindy Options:\n\n";
   print "-L <language>\tUse <language>.\n";
   print "-x <file>\tFull path to xindy executable.\n",
    "\t\t(Default assumes xindy is on the operating system's path.)\n";

   print "\nMakeindex Options:\n";
   print "(See makeindex documentation for further details on these ";
   print "options.)\n\n";
   print "-c\t\tCompress intermediate blanks.\n";
   print "-g\t\tEmploy German word ordering.\n";
   print "-p <num>\tSet the starting page number to be <num>.\n";
   print "-r\t\tDisable implicit page range formation.\n";
   print "-m <file>\tFull path to makeindex executable.\n",
    "\t\t(Default assumes makeindex is on the operating system's path.)\n";
}

sub VERSION_MESSAGE{

   my $verYear = '';

   if ($version=~/(\d{4})-\d{2}-\d{2}/)
   {
      $verYear = "-$1";
   }

   print "Makeglossaries Version $version\n";
   print "Copyright (C) 2007$verYear Nicola L C Talbot\n";
   print "This material is subject to the LaTeX Project Public License.\n";
}

1;

=head1 NAME

makeglossaries  - Calls makeindex/xindy for LaTeX documents using glossaries package

=head1 SYNOPSIS

B<makeglossaries> [B<-o> I<file>] [B<-q>] [B<-Q>] [B<-k>] [B<-n>]
[B<-s> I<file>] [B<-t> I<file>] [B<-L> I<language>] [B<-c>] [B<-g>] [B<-l>]
[B<-p> I<num>] [B<-r>] [B<-d> I<aux dir>] [B<-m> I<file>] [B<-x> I<file>]
[B<--version>] [B<--help>] I<basename>

=head1 DESCRIPTION

B<makeglossaries> is designed for use with LaTeX documents that
use the glossaries package. The mandatory argument I<basename> should
be the name of the LaTeX document without the .tex extension. 
B<makeglossaries> will read the auxiliary file to determine whether
B<makeindex> or B<xindy> should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to B<makeglossaries>.

=head1 OPTIONS

=over 4

=item B<-q>

Quiet mode. Reduces chatter to standard output.

=item B<-Q>

Silences warning about being unable to fork.

=item B<-k>

Don't try forking with piped redirection. (Lessens the
effect of -q)

=item B<-n>

Print the commands that would normally be executed but don't run them.

=item B<-o> I<file>

Use I<file> as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)

=item B<-s> I<file>

Use I<file> as the style file. Note that if you use this option,
you need to know whether B<makeindex> or B<xindy> will be called, as
they have different style files.

=item B<-t> I<file>

Use I<file> as the transcript file.

=item B<-l>

Letter ordering.

=item B<-L> I<language>

This option only has an effect if B<xindy> is called. Sets the
language. See B<xindy> documentation for further details.

=item B<-c>

Compress intermediate blanks (B<makeindex> only).

=item B<-g>

Employ German word ordering (B<makeindex> only).

=item B<-p> I<num>

Sets the starting page number to be I<num> (B<makeindex> only).

=item B<-r>

Disable implicit page range formation (B<makeindex> only).

=item B<-d> I<aux dir>

Specify the directory the .aux, .glo etc files are located.
Defaults to the parent directory of the base file I<filename>.

=item B<-m> I<file>

Specify the full path name for B<makeindex> to I<file> in the 
event that B<makeindex> isn't on the operating system's path.

=item B<-x> I<file>

Specify the full path name for B<xindy> to I<file> in the 
event that B<xindy> isn't on the operating system's path.

=item B<--version>

Prints version number and exits.

=item B<--help>

Prints help message and exits.

=back

=head1 REQUIRES

Perl, Getopt::Std, and makeindex or xindy (depending on glossaries
package options).

=head1 LICENSE

This is free software distributed under the LaTeX Project Public 
License. There is NO WARRANTY.
See L<http://www.latex-project.org/lppl.txt> for details.

=head1 AUTHOR

Nicola L. C. Talbot,
L<http://www.dickimaw-books.com/>

=head1 RECOMMENDED READING

The glossaries manual:

	texdoc glossaries

=cut

